Knowledge Is Flat: A Seq2Seq Generative Framework for Various Knowledge Graph Completion

Knowledge Graph Completion (KGC) has been recently extended to multiple knowledge graph (KG) structures, initiating new research directions, e.g. static KGC, temporal KGC and few-shot KGC. Previous works often design KGC models closely coupled with specific graph structures, which inevitably results in two drawbacks: 1) structure-specific KGC models are mutually incompatible; 2) existing KGC methods are not adaptable to emerging KGs. In this paper, we propose KG-S2S, a Seq2Seq generative framework that could tackle different verbalizable graph structures by unifying the representation of KG facts into "flat" text, regardless of their original form. To remedy the KG structure information loss from the "flat" text, we further improve the input representations of entities and relations, and the inference algorithm in KG-S2S. Experiments on five benchmarks show that KG-S2S outperforms many competitive baselines, setting new state-of-the-art performance. Finally, we analyze KG-S2S's ability on the different relations and the Non-entity Generations.

==> tables/Comparasion_of_parameters.tex <==
\begin{table*}[!htbp]
	\centering
	\begin{tabular}{lcccc}
		\toprule
        &MRR &H@1 &H@10 &params  \\
		\midrule
KG-BERTBERT-base &.216 &.041 &.524 &110M \\
StARBERT-base &.364 &.222 &.647 &110M \\
KG-BERTRoBERTa-base &.278 &.130 &.636 &123M\\
StARRoBERTa-base &.343 &.202 &.621 &123M\\
KG-BERTRoBERTa-large &.297 &.119 &.698 &354M\\
StARRoBERTa-large &.401 &.243 &\textbf{.709} &354M\\
\midrule
\method T5-small &.550 &.520 &.607 &60M\\
\method T5-base &\textbf{.577} &\textbf{.534} &.658 &220M\\
\bottomrule
\end{tabular}
\caption{Comparisons with KG-BERT on \datawnrr }
\label{tab:comparsion on number of parameters} 
\end{table*}
